Long-term Pedestrian Trajectory Prediction using Mutable Intention Filter and Warp LSTM

Trajectory prediction is one of the key capabilities for robots to safely navigate and interact with pedestrians. Critical insights from human intention and behavioral patterns need to be integrated to effectively forecast long-term pedestrian behavior. Thus, we propose a framework incorporating a Mutable Intention Filter and a Warp LSTM (MIF-WLSTM) to simultaneously estimate human intention and perform trajectory prediction. The Mutable Intention Filter is inspired by particle filtering and genetic algorithms, where particles represent intention hypotheses that can be mutated throughout the pedestrian motion. Instead of predicting sequential displacement over time, our Warp LSTM learns to generate offsets on a full trajectory predicted by a nominal intention-aware linear model, which considers the intention hypotheses during filtering process. Through experiments on a publicly available dataset, we show that our method outperforms baseline approaches and demonstrate the robust performance of our method under abnormal intention-changing scenarios. Code is available at https://github.com/tedhuang96/mifwlstm.

==> bib_backup_jun_26.tex <==
% Proc. IEEE Comput. Soc. Conf. Comput. Vis. Pattern Recognit.


@article{helbing1995social,
  title={Social force model for pedestrian dynamics},
  author={Helbing, Dirk and Molnar, Peter},
  journal={Phys. Rev. E},
  volume={51},
  number={5},
  pages={4282},
  year={1995},
  publisher={APS}
}

@inproceedings{gupta2018social,
  title={Social gan: Socially acceptable trajectories with generative adversarial networks},
  author={Gupta, Agrim and Johnson, Justin and Fei-Fei, Li and Savarese, Silvio and Alahi, Alexandre},
  booktitle=CVPR,
  pages={2255--2264},
  year={2018}
}

@inproceedings{vemula2018social,
  title={Social attention: Modeling attention in human crowds},
  author={Vemula, Anirudh and Muelling, Katharina and Oh, Jean},
  booktitle=ICRA,
  pages={1--7},
  year={2018},
  organization={IEEE}
}

@inproceedings{alahi2016social,
  title={Social lstm: Human trajectory prediction in crowded spaces},
  author={Alahi, Alexandre and Goel, Kratarth and Ramanathan, Vignesh and Robicquet, Alexandre and Fei-Fei, Li and Savarese, Silvio},
  booktitle=CVPR,
  pages={961--971},
  year={2016}
}

@article{graves2013generating,
  title={Generating sequences with recurrent neural networks},
  author={Graves, Alex},
  journal={arXiv preprint arXiv:1308.0850},
  year={2013}
}

@inproceedings{ivanovic2019trajectron,
  title={The Trajectron: Probabilistic multi-agent trajectory modeling with dynamic spatiotemporal graphs},
  author={Ivanovic, Boris and Pavone, Marco},
  booktitle=ICCV,
  pages={2375--2384},
  year={2019}
}

@inproceedings{particke2018improvements,
  title={Improvements in pedestrian movement prediction by considering multiple intentions in a multi-hypotheses filter},
  author={Particke, Florian and Hiller, Markus and Feist, Christian and Thielecke, J{\"o}rn},
  booktitle={Proc. IEEE/ION Pos. Loc. Nav. Symp.},
  pages={209--212},
  year={2018},
  organization={IEEE}
}

@inproceedings{particke2017pedestrian,
  title={Pedestrian Tracking using a Generalized Potential Field Approach},
  author={Particke, Florian and Patino-Studencki, Lucila and Thielecke, J{\"o}rn and Feist, Christian},
  booktitle={VISIGRAPP (6: VISAPP)},
  pages={509--514},
  year={2017}
}

@incollection{bandyopadhyay2013intention,
  title={Intention-aware motion planning},
  author={Bandyopadhyay, Tirthankar and Won, Kok Sung and Frazzoli, Emilio and Hsu, David and Lee, Wee Sun and Rus, Daniela},
  booktitle={Algo. Fdn. Rob. X},
  pages={475--491},
  year={2013},
  publisher={Springer}
}


@article{du2019online,
  title={Online monitoring for safe pedestrian-vehicle interactions},
  author={Du, Peter and Huang, Zhe and Liu, Tianqi and Xu, Ke and Gao, Qichao and Sibai, Hussein and Driggs-Campbell, Katherine and Mitra, Sayan},
  journal={arXiv preprint arXiv:1910.05599},
  year={2019}
}

@inproceedings{dragan2013legibility,
  title={Legibility and predictability of robot motion},
  author={Dragan, Anca D and Lee, Kenton CT and Srinivasa, Siddhartha S},
  booktitle=HRI,
  pages={301--308},
  year={2013},
  organization={IEEE}
}

@inproceedings{chen2017socially,
  title={Socially aware motion planning with deep reinforcement learning},
  author={Chen, Yu Fan and Everett, Michael and Liu, Miao and How, Jonathan P},
  booktitle=IROS,
  pages={1343--1350},
  year={2017},
  organization={IEEE}
}

@inproceedings{carvalho2019long,
  title={Long-term Prediction of Motion Trajectories Using Path Homology Clusters},
  author={Carvalho, J Frederico and Vejdemo-Johansson, Mikael and Pokorny, Florian T and Kragic, Danica},
  booktitle=IROS,
  pages={765--772},
  year={2019},
  organization={IEEE}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle=CVPR,
  pages={770--778},
  year={2016}
}

@article{majecka2009statistical,
  title={Statistical models of pedestrian behaviour in the forum},
  author={Majecka, Barbara},
  journal={Master's thesis, School of Informatics, University of Edinburgh},
  year={2009},
  publisher={Citeseer}
}

@inproceedings{hug2018particle,
  title={Particle-based pedestrian path prediction using LSTM-MDL models},
  author={Hug, Ronny and Becker, Stefan and H{\"u}bner, Wolfgang and Arens, Michael},
  booktitle=ITSC,
  pages={2684--2691},
  year={2018},
  organization={IEEE}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@inproceedings{pellegrini2009you,
  title={You'll never walk alone: Modeling social behavior for multi-target tracking},
  author={Pellegrini, Stefano and Ess, Andreas and Schindler, Konrad and Van Gool, Luc},
  booktitle=ICCV,
  pages={261--268},
  year={2009},
  organization={IEEE}
}

@inproceedings{zhang2019sr,
  title={Sr-lstm: State refinement for lstm towards pedestrian trajectory prediction},
  author={Zhang, Pu and Ouyang, Wanli and Zhang, Pengfei and Xue, Jianru and Zheng, Nanning},
  booktitle=CVPR,
  pages={12085--12094},
  year={2019}
}

@inproceedings{xu2018encoding,
  title={Encoding crowd interaction with deep neural network for pedestrian trajectory prediction},
  author={Xu, Yanyu and Piao, Zhixin and Gao, Shenghua},
  booktitle=CVPR,
  pages={5275--5284},
  year={2018}
}

@inproceedings{bartoli2018context,
  title={Context-aware trajectory prediction},
  author={Bartoli, Federico and Lisanti, Giuseppe and Ballan, Lamberto and Del Bimbo, Alberto},
  booktitle=ICPR,
  pages={1941--1946},
  year={2018},
  organization={IEEE}
}

@inproceedings{sadeghian2019sophie,
  title={Sophie: An attentive gan for predicting paths compliant to social and physical constraints},
  author={Sadeghian, Amir and Kosaraju, Vineet and Sadeghian, Ali and Hirose, Noriaki and Rezatofighi, Hamid and Savarese, Silvio},
  booktitle=CVPR,
  pages={1349--1358},
  year={2019}
}

@article{salzmann2020trajectron++,
  title={Trajectron++: Multi-Agent Generative Trajectory Forecasting With Heterogeneous Data for Control},
  author={Salzmann, Tim and Ivanovic, Boris and Chakravarty, Punarjay and Pavone, Marco},
  journal={arXiv preprint arXiv:2001.03093},
  year={2020}
}

@incollection{van2011reciprocal,
  title={Reciprocal n-body collision avoidance},
  author={Van Den Berg, Jur and Guy, Stephen J and Lin, Ming and Manocha, Dinesh},
  booktitle={Rob. Res.},
  pages={3--19},
  year={2011},
  publisher={Springer}
}

@inproceedings{yamaguchi2011you,
  title={Who are you with and where are you going?},
  author={Yamaguchi, Kota and Berg, Alexander C and Ortiz, Luis E and Berg, Tamara L},
  booktitle=CVPR,
  pages={1345--1352},
  year={2011},
  organization={IEEE}
}

@inproceedings{kuderer2012feature,
  title={Feature-based prediction of trajectories for socially compliant navigation},
  author={Kuderer, Markus and Kretzschmar, Henrik and Sprunk, Christoph and Burgard, Wolfram},
  booktitle=RSS,
  year={2012}
}

@article{fernando2018soft+,
  title={Soft+ hardwired attention: An lstm framework for human trajectory prediction and abnormal event detection},
  author={Fernando, Tharindu and Denman, Simon and Sridharan, Sridha and Fookes, Clinton},
  journal={Neural Netw.},
  volume={108},
  pages={466--478},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{chen2017socially,
  title={Socially aware motion planning with deep reinforcement learning},
  author={Chen, Yu Fan and Everett, Michael and Liu, Miao and How, Jonathan P},
  booktitle=IROS,
  pages={1343--1350},
  year={2017},
  organization={IEEE}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural Comput.},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

@article{chung2014empirical,
  title={Empirical evaluation of gated recurrent neural networks on sequence modeling},
  author={Chung, Junyoung and Gulcehre, Caglar and Cho, KyungHyun and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1412.3555},
  year={2014}
}

@article{rudenko2019human,
  title={Human motion trajectory prediction: A survey},
  author={Rudenko, Andrey and Palmieri, Luigi and Herman, Michael and Kitani, Kris M and Gavrila, Dariu M and Arras, Kai O},
  journal={arXiv preprint arXiv:1905.06113},
  year={2019}
}

@inproceedings{volz2016data,
  title={A data-driven approach for pedestrian intention estimation},
  author={V{\"o}lz, Benjamin and Behrendt, Karsten and Mielenz, Holger and Gilitschenski, Igor and Siegwart, Roland and Nieto, Juan},
  booktitle=ITSC,
  pages={2607--2612},
  year={2016},
  organization={IEEE}
}

@inproceedings{rasouli2019pie,
  title={PIE: A Large-Scale Dataset and Models for Pedestrian Intention Estimation and Trajectory Prediction},
  author={Rasouli, Amir and Kotseruba, Iuliia and Kunic, Toni and Tsotsos, John K},
  booktitle=ICCV,
  pages={6262--6271},
  year={2019}
}

@inproceedings{xue2017bi,
  title={Bi-prediction: pedestrian trajectory prediction based on bidirectional LSTM classification},
  author={Xue, Hao and Huynh, Du Q and Reynolds, Mark},
  booktitle={2017 International Conference on Digital Image Computing: Techniques and Applications (DICTA)},
  pages={1--8},
  year={2017},
  organization={IEEE}
}

@inproceedings{rehder2015goal,
  title={Goal-directed pedestrian prediction},
  author={Rehder, Eike and Kloeden, Horst},
  booktitle=ICCVW,
  pages={50--58},
  year={2015}
}


@inproceedings{karasev2016intent,
  title={Intent-aware long-term prediction of pedestrian motion},
  author={Karasev, Vasiliy and Ayvaci, Alper and Heisele, Bernd and Soatto, Stefano},
  booktitle=ICRA,
  pages={2543--2549},
  year={2016},
  organization={IEEE}
}

@article{katyalintent,
  title={Intent-Aware Pedestrian Prediction for Adaptive Crowd Navigation},
  author={Katyal, Kapil D and Hager, Gregory D and Huang, Chien-Ming}
}

@inproceedings{ghori2018learning,
  title={Learning to forecast pedestrian intention from pose dynamics},
  author={Ghori, Omair and Mackowiak, Radek and Bautista, Miguel and Beuter, Niklas and Drumond, Lucas and Diego, Ferran and Ommer, Bj{\"o}rn},
  booktitle=IV,
  pages={1277--1284},
  year={2018},
  organization={IEEE}
}


@article{prakash2016neural,
  title={Neural paraphrase generation with stacked residual lstm networks},
  author={Prakash, Aaditya and Hasan, Sadid A and Lee, Kathy and Datla, Vivek and Qadir, Ashequl and Liu, Joey and Farri, Oladimeji},
  journal={arXiv preprint arXiv:1610.03098},
  year={2016}
}


@article{kim2017residual,
  title={Residual LSTM: Design of a deep recurrent architecture for distant speech recognition},
  author={Kim, Jaeyoung and El-Khamy, Mostafa and Lee, Jungwon},
  journal={arXiv preprint arXiv:1701.03360},
  year={2017}
}

@article{kim2018residual,
  title={Residual LSTM attention network for object tracking},
  author={Kim, Hong-In and Park, Rae-Hong},
  journal={Ieee Signal Processing Letters},
  volume={25},
  number={7},
  pages={1029--1033},
  year={2018},
  publisher={IEEE}
}

@article{wang2018using,
  title={Using a stacked residual LSTM model for sentiment intensity prediction},
  author={Wang, Jin and Peng, Bo and Zhang, Xuejie},
  journal={Neurocomputing},
  volume={322},
  pages={93--101},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{huang2017improved,
  title={An improved residual LSTM architecture for acoustic modeling},
  author={Huang, Lu and Xu, Ji and Sun, Jiasong and Yang, Yi},
  booktitle={2017 2nd International Conference on Computer and Communication Systems (ICCCS)},
  pages={101--105},
  year={2017},
  organization={IEEE}
}

@article{tran2017named,
  title={Named entity recognition with stack residual lstm and trainable bias decoding},
  author={Tran, Quan and MacKinlay, Andrew and Yepes, Antonio Jimeno},
  journal={arXiv preprint arXiv:1706.07598},
  year={2017}
}

@inproceedings{wang2016recurrent,
  title={Recurrent residual learning for sequence classification},
  author={Wang, Yiren and Tian, Fei},
  booktitle={Proceedings of the 2016 conference on empirical methods in natural language processing},
  pages={938--943},
  year={2016}
}

@inproceedings{xu2017image,
  title={Image captioning with deep LSTM based on sequential residual},
  author={Xu, Kaisheng and Wang, Hanli and Tang, Pengjie},
  booktitle={2017 IEEE International Conference on Multimedia and Expo (ICME)},
  pages={361--366},
  year={2017},
  organization={IEEE}
}

@article{zhao2018deep,
  title={Deep residual bidir-LSTM for human activity recognition using wearable sensors},
  author={Zhao, Yu and Yang, Rennong and Chevalier, Guillaume and Xu, Ximeng and Zhang, Zhenxing},
  journal={Mathematical Problems in Engineering},
  volume={2018},
  year={2018},
  publisher={Hindawi}
}

@inproceedings{schneider2013pedestrian,
  title={Pedestrian path prediction with recursive bayesian filters: A comparative study},
  author={Schneider, Nicolas and Gavrila, Dariu M},
  booktitle={German Conf. on Pattern Recogn.},
  pages={174--183},
  year={2013},
  organization={Springer}
}

@inproceedings{schulz2015controlled,
  title={A controlled interactive multiple model filter for combined pedestrian intention recognition and path prediction},
  author={Schulz, Andreas T and Stiefelhagen, Rainer},
  booktitle=ITSC,
  pages={173--178},
  year={2015},
  organization={IEEE}
}

@inproceedings{kitani2012activity,
  title={Activity forecasting},
  author={Kitani, Kris M and Ziebart, Brian D and Bagnell, James Andrew and Hebert, Martial},
  booktitle={European Conference on Computer Vision},
  pages={201--214},
  year={2012},
  organization={Springer}
}

@inproceedings{ziebart2009planning,
  title={Planning-based prediction for pedestrians},
  author={Ziebart, Brian D and Ratliff, Nathan and Gallagher, Garratt and Mertz, Christoph and Peterson, Kevin and Bagnell, J Andrew and Hebert, Martial and Dey, Anind K and Srinivasa, Siddhartha},
  booktitle=IROS,
  pages={3931--3936},
  year={2009},
  organization={IEEE}
}

@inproceedings{particke2018entropy,
  title={Entropy-Based Intention Change Detection with a Multi-Hypotheses Filter},
  author={Particke, Florian and Hofmann, Christian and Hiller, Markus and Bey, Henrik and Feist, Christian and Thielecke, J{\"o}rn},
  booktitle={2018 21st International Conference on Information Fusion (FUSION)},
  pages={610--616},
  year={2018},
  organization={IEEE}
}

@article{baldwin2001discerning,
  title={Discerning intentions in dynamic human action},
  author={Baldwin, Dare A and Baird, Jodie A},
  journal={Trends Cogn. Sci.},
  volume={5},
  number={4},
  pages={171--178},
  year={2001},
  publisher={Elsevier}
}

@inproceedings{becker2018red,
  title={Red: A simple but effective baseline predictor for the trajnet benchmark},
  author={Becker, Stefan and Hug, Ronny and Hubner, Wolfgang and Arens, Michael},
  booktitle=ECCV,
  pages={0--0},
  year={2018}
}

@article{lipton2015critical,
  title={A critical review of recurrent neural networks for sequence learning},
  author={Lipton, Zachary C and Berkowitz, John and Elkan, Charles},
  journal={arXiv preprint arXiv:1506.00019},
  year={2015}
}
